First-Order logic and its Infinitary Quantifier Extensions over Countable Words

We contribute to the refined understanding of the language-logic-algebra interplay in the context of first-order properties of countable words. We establish decidable algebraic characterizations of one variable fragment of FO as well as boolean closure of existential fragment of FO via a strengthening of Simon's theorem about piecewise testable languages. We propose a new extension of FO which admits infinitary quantifiers to reason about the inherent infinitary properties of countable words. We provide a very natural and hierarchical block-product based characterization of the new extension. We also explicate its role in view of other natural and classical logical systems such as WMSO and FO[cut] - an extension of FO where quantification over Dedekind-cuts is allowed. We also rule out the possibility of a finite basis for a block-product based characterization of these logical systems. Finally, we report simple but novel algebraic characterizations of one variable fragments of the hierarchies of the new proposed extension of FO.

==> app.tex <==
%! TEX root = main.tex

\begin{lemma}\label{lem:eqcontent}
	Let $M$ be a commutative, shuffle-idempotent o-algebra with the property $\{m_1, \ldots,
m_k\}^\kappa = m_1^\kappa \ldots m_k^\kappa$, and let $h \colon \Sigma^\circ \to M$
be a morphism to this o-monoid. Then for any countable word $u$, 
\[ h(u) = \prod_{a \in \mathrm{alph}(u)} h(a) \]
where $\mathrm{alph}(u) \subseteq \Sigma$ is the set of letters in $u$.
\end{lemma}
\begin{proof}
We only need to show that the algebra operations preserve this property. For $u, v \in
\Sigma^\circ$, if $h(u)$ and $h(v)$ satisfy the property, then clearly $h(u).h(v)$ does.
Since every element is an ordinal idempotent as well as an ordinal-star idempotent, for
any $u \in \Sigma^\circ$, it's clear that $(h(u))^\tau$ and $(h(u))^{\tau^*}$ satisfy the
properties. Finally, the shuffle case reduces to the concatenation case because of the
shuffle properties.
\end{proof}


\begin{theorem} \label{fo1-app}
Let $L \subseteq \Sigma^\circ$ be a language. The following are equivalent.
\begin{enumerate}
	\item $L$ is recognized by commutative, shuffle-idempotent o-algebra with the
		property $\{m_1, \ldots, m_k\}^\kappa = m_1^\kappa \ldots m_k^\kappa$.
	\item $L$ is a boolean combination of languages of the form $A^\circ$ where $A
		\subseteq \Sigma$.
	\item $L$ is definable in $\mathrm{FO}^1$.
	\item $L$ is recognized by direct product of $U_1$s.
\end{enumerate}
\end{theorem}
\begin{proof}
	($1 \Rightarrow 2$) Let $L$ be recognized by $h \colon \Sigma^\circ \to M$ where
	$M$ is commutative, shuffle-idempotent and has the property $\{m_1, \ldots,
	m_k\}^\kappa = m_1^\kappa\ldots m_k^\kappa$. By Lemma~\ref{lem:eqcontent}, $L$ is
	union of equivalence classes defined by the relation $\{(u,v) \mid \mathrm{alph}(u) =
	\mathrm{alph}(v)\}$. All these classes are boolean combination of languages of the
	form $A^\circ$ for some $A \subseteq \Sigma$, as seen below.
	\[ \{u \mid \mathrm{alph}(u)=A \} = A^\circ \setminus \left ( \bigcup_{b \in A}
	(A \setminus \{b\})^\circ \right ) \]
	
	($2 \Rightarrow 3$) Note that $A^\circ$ is expressed by the $\mathrm{FO}^1$
	formula $\forall x. \lor_{a \in A} a(x)$. Rest follows from boolean closure of
	$\mathrm{FO}^1$.

	($3 \Rightarrow 4$) Due to the restriction of a single variable, any formula
	$\phi(x)$ is just a boolean combination of atomic letter predicates. In fact,
	since any position can have exactly one letter, we can consider $\phi(x)$ to be
	just a disjunction of the letter predicates. A language defined by $\exists x.
	a(x)$ is recognized by the o-monoid $U_1$. A language defined by boolean
	combination of such sentences can be recognized by direct product of $U_1$s.

	($4 \Rightarrow 1$) The monoid $U_1$ satisfies the properties mentioned, and the
	properties are preserved under direct product.
\end{proof}

\begin{theorem}
Let $L \subseteq \Sigma^\circ$ be a language. The following are equivalent.
\begin{enumerate}
	\item $L$ is recognized by $\jc$-trivial o-algebra with every idempotent being
		shuffle-idempotent.
	\item $L$ is recognized by $\Sigma^\circ / \sim_n$ for some $n$.
	\item $L$ is definable in $\bs$.
\end{enumerate}
%
\end{theorem}
\begin{proof}[sketch]
$(1 \Rightarrow 2)$ Let $L$ be recognized by $h \colon \Sigma^\circ \to M$ where $M$ is
$\jc$-trivial with every idempotent being shuffle idempotent. Let the maximal length of
strict $<_\jc$-chains in $M$ be $n$. We have to show $u \sim_{2n-1} v$ implies $h(u) =
h(v)$. By Lemma~\ref{lem:fin} there exists finite words $\hat{u} \sim_{2n-1} u$ and
$\hat{v} \sim_{2n-1} v$. By the classical results, $h(\hat{u}) = h(\hat{v})$. Next we
show, if $u'$ is a finite subword of $u$ and $u' \sim_{2n-1} u$, then $h(u) = h(u')$.
This part needs evaluation tree.

$(2 \Rightarrow 1)$ By properties of $\sim_n$, ...

$(2 \Rightarrow 3)$ obvious.

$(3 \Rightarrow 2)$ Looks intuitive. If $u \sim_n v$, then a $\bs$ formula with $n$
variables should not be able to distinguish them.
\end{proof}

The syntax of the new logic is given by 
\[ a(x) \mid x < y \mid \neg \varphi \mid \varphi \vee \varphi \mid \exists x ~\varphi 
\mid \exists^{\omega^n} x ~\varphi \mid \exists^{\omega*^n} x ~\varphi 
\mid \exists^{\delta^n} ~\varphi \]
Let $\mathrm{free} (\varphi)$ be the set of free variables of $\varphi$ and 
$\mathcal{A}$ be an 
assignment of $\mathrm{free} (\varphi)$ to positions in a countable word $w$. 
Then $w, 
\mathcal{A}$ is a model of $\varphi$ if it satisifies the conditions
below:
\begin{align*}
w,\mathcal{A} & \models a(x) &&\text{ iff }\mathcal{A}(x)\text{ is labelled }
 a\in \Sigma \\
w,\mathcal{A} & \models x < y &&\text{ iff }\mathcal{A}(x) < \mathcal{A}(y) \\
w,\mathcal{A} & \models \neg \varphi &&\text{ iff }w,\mathcal{A} \not \models \varphi \\
w,\mathcal{A} & \models \varphi \vee \psi &&\text{ iff } w,\mathcal{A} \models \varphi 
\text{ or } w,\mathcal{A} \models \psi \\
w,\mathcal{A}  & \models \exists x ~\varphi &&\text{ iff there
	exists $i$ 
such that } w,\mathcal{A}[x=i] \models \varphi \\
	w,\mathcal{A} & \models \exists^{\omega^n} x~\varphi &&\begin{aligned}[t]
	\text{ iff }& \{i \in \mathrm{dom}(w) \mid w, \mathcal{A}[x=i] \models \varphi \}\\
		    &  \text{has a subordering of type } \omega^n 
\end{aligned} \\
	w,\mathcal{A} & \models \exists^{\omega*^n} x~\varphi &&\begin{aligned}[t]
	\text{ iff }& \{i \in \mathrm{dom}(w) \mid w, \mathcal{A}[x=i] \models \varphi \}\\
		    &  \text{has a subordering of type } \omega*^n 
\end{aligned} \\
	w,\mathcal{A} & \models \exists^{\delta^n} x~\varphi &&\begin{aligned}[t]
	\text{ iff }& \{i \in \mathrm{dom}(w) \mid w, \mathcal{A}[x=i] \models \varphi \}\\
		    &  \text{has rank } \geq n
\end{aligned} 
%w,\mathcal{A} & \models \exoms x~\phi &&\begin{aligned}[t]
%	\text{ iff }& \text{ there exists an $\omega^*$-sequence
%	of positions} \\
%&  \ldots,x_2, x_1 \text{ s.t. } w,\mathcal{A}[x=x_i] \models
%\phi ~~\forall i 
%\end{aligned}
\end{align*}

We'll use relativisation in our new logic and so we prove in the
following lemma that this works as intended.

\begin{lemma}
For any $\phi$ in the generalized FO logic, we can construct a relativised formula
$\phi_{<x}$, where $x \notin \mathrm{free}(\phi)$, such that for any word $w$ with
assignment
$\mathcal{A}$ 
\[ w, \mathcal{A}[x=i] \models \phi_{<x} \text{ iff } w_{<i}, \mathcal{A} \models \phi \]
\end{lemma}

\begin{proof}
Proof is via structural induction on generalized FO formula. We only show the
case for the $\exists^{\omega^n}$ quantifier. Let $\phi = \exists^{\omega^n} y \psi$.
\begin{align*}
	& w_{<i}, \mathcal{A} \models \exists^{\omega^n} y ~\psi \\
	& \begin{aligned} \iff \exists \text{ a subordering } S \subseteq 
		\mathrm{dom}(w_{<i}) &\text{ of order type } \omega^n \text{ such that }\\
		& w_{<i}, \mathcal{A}[y=j] \models \psi ~~\forall j \in S 
	\end{aligned} \\
	& \begin{aligned} \iff \exists \text{ a subordering }& S \subseteq 
		\mathrm{dom}(w) \text{ of order type } \omega^n \text{ such that }\\
	& w_{<i}, \mathcal{A}[y=j] \models \psi \text{ and } j < i ~~\forall j \in S 
	\end{aligned} \\
	& \begin{aligned} \iff \exists \text{ a subordering }& S \subseteq 
		\mathrm{dom}(w) \text{ of order type } \omega^n \text{ such that }\\
        & w, \mathcal{A}[x=i,y=j] \models \psi_{<x} \text{ and } j < i ~~\forall j \in S 
	\end{aligned} \\
	& \iff w, \mathcal{A}[x=i] \models \exists^{\omega^n} y ( \psi_{<x} 
	\wedge y < x)
\end{align*}
\end{proof}

\subsection{Chain o-alegbras}
\label{subsec:chain}

For each natural number $n$, we define commutative and
idempotent o-algebras
$\Omega_n$, $\Omega^*_n$ and $\Delta_n$ as follows.

$\Omega_n = \{ 1, a^{\omega^0}, a^{\omega^1}, \ldots, a^{\omega^n}\}$ where and for any $0
\leq k < n$, we have $(a^{\omega^k})^\tau = a^{\omega^{k+1}}$. Every element is an
ordinal* idempotent; in particular, $1$ and $a^{\omega^n}$ are shuffle idempotents.

$\Omega^*_n = \{ 1, a^{{\omega^*}^0}, a^{{\omega^*}^1}, \ldots, a^{{\omega^*}^n}\}$ where
for any $0 \leq k < n$, we have $(a^{{\omega^*}^k})^{\tau^*} =
a^{{\omega^*}^{k+1}}$. Every element is an ordinal idempotent; in particular, $1$ and
$a^{{\omega^*}^n}$ are shuffle idempotents.

$\Delta_n = \{ 1, a^{\delta^0}, a^{\delta^1}, \ldots, a^{\delta^n}\}$ where for any 
$0 \leq k < n$, we have $(a^{\delta^k})^\tau= (a^{\delta^k})^{\tau^*}
= a^{\delta^{k+1}}$. Here $1$ and $a^{\delta^n}$ are shuffle idempotents.
%\begin{figure}[h] \centering \input{chain.tikz} \caption{The o-algebra $I_n$}
%\label{fig:chain-algebra} \end{figure}
%\begin{figure}[h!]
%	%\centering
%	\begin{subfigure}[t]{0.33\textwidth}
%	%	\centering
%		\begin{tikzpicture}
%		\node at (0,0) {$1$};
%		\draw[thick] (-0.3, -0.3) rectangle (0.3, 0.3);
%		\node at (0,-0.7) {$a^{\omega^0}$};
%		\draw[thick] (-0.3, -1) rectangle (0.3, -0.4);
%		\node at (0,-1.4) {$a^{\omega^1}$};
%		\draw[thick] (-0.3, -1.7) rectangle (0.3, -1.1);
%		\node at (0,-1.9) [circle, fill, inner sep=1pt] {};
%		\node at (0,-2.1) [circle, fill, inner sep=1pt] {};
%		\node at (0,-2.6) {$a^{\omega^n}$};
%		\draw[thick] (-0.3, -2.9) rectangle (0.3, -2.3);
%		\end{tikzpicture}
%	\caption{The o-algebra $\Omega_n$}
%	\end{subfigure}%
%	\begin{subfigure}[t]{0.33\textwidth}
%	%	\centering
%		\begin{tikzpicture}
%		\node at (0,0) {$1$};
%		\draw[thick] (-0.3, -0.3) rectangle (0.3, 0.3);
%		\node at (0,-0.7) {$a^{{\omega^*}^0}$};
%		\draw[thick] (-0.3, -1) rectangle (0.3, -0.4);
%		\node at (0,-1.4) {$a^{{\omega^*}^1}$};
%		\draw[thick] (-0.3, -1.7) rectangle (0.3, -1.1);
%		\node at (0,-1.9) [circle, fill, inner sep=1pt] {};
%		\node at (0,-2.1) [circle, fill, inner sep=1pt] {};
%		\node at (0,-2.6) {$a^{{\omega^*}^n}$};
%		\draw[thick] (-0.3, -2.9) rectangle (0.3, -2.3);
%		\end{tikzpicture}
%	\caption{The o-algebra $\Omega^*_n$}
%	\end{subfigure}
%	\begin{subfigure}[t]{0.33\textwidth}
%	%	\centering
%		\begin{tikzpicture}
%		\node at (0,0) {$1$};
%		\draw[thick] (-0.3, -0.3) rectangle (0.3, 0.3);
%		\node at (0,-0.7) {$a^{\delta^0}$};
%		\draw[thick] (-0.3, -1) rectangle (0.3, -0.4);
%		\node at (0,-1.4) {$a^{\delta^1}$};
%		\draw[thick] (-0.3, -1.7) rectangle (0.3, -1.1);
%		\node at (0,-1.9) [circle, fill, inner sep=1pt] {};
%		\node at (0,-2.1) [circle, fill, inner sep=1pt] {};
%		\node at (0,-2.6) {$a^{\delta^n}$};
%		\draw[thick] (-0.3, -2.9) rectangle (0.3, -2.3);
%		\end{tikzpicture}
%	\caption{The o-algebra $\Delta_n$}
%	\end{subfigure}
%	\caption{Chain algebra}
%	\label{fig:chain-algebra}
%\end{figure}

It's clear that the $\mathcal{J}$-classes in all three algebra are singleton and form a
chain as shown in Figure~\ref{fig:chain-algebra}.

\begin{lemma}\label{lem:chain-inside-logic} 
	The o-algebras $\Omega_n$, $\Omega^*_n$ and $\Delta_n$ satisfy FO-CUT equations.
	Additionally,  $\Delta_n$ satisfy WMSO equations. 
\end{lemma}

Let $\mathrm{FO}[\exists^{\omega^n}]$ denote the generalized FO logic with
$\exists^{\omega^i}$ quantifiers for $1 \leq i \leq n$. Let
$\mathrm{FO}[\exists^\omega_\mathbb{N}]$ denote the generalized FO logic with 
quantifiers $\exists^{\omega^i}$ for $1 \leq i$. 
\begin{lemma}\label{lem:singleomega}
	Languages recognized by $\Omega_n$ are definable in
	$\mathrm{FO}[\exists^{\omega^n}]$ with one variable.
\end{lemma}
\begin{proof}
	The proof is via the usual approach of induction on the $\mathcal{J}$ class order.
	We express any $\mathcal{J}$ class drop inside $\Omega_n$ using the appropriate
	logic with 1 variable. The rest follow easily. Suppose the $\mathcal{J}$ class
	under consideration is that of $a^{\omega^i}$ where $0 \leq i < n$. By induction
	hypothesis, let the $\mathcal{J}$ class drop for the higher element
	$a^{\omega^{i-1}}$ be a disjunction of $\mathrm{FO}^1[\exists^{\omega^{i-1}}]$
	sentences of the form $\exists^{\omega^j} x . c(x)$ where $c \in \Sigma$ and $0
	\leq j \leq i-1$ with $\exists^{\omega^0}$ being just the normal FO existential
	quantifier.

	The current $\mathcal{J}$ class drop can happen due to letter witness, omega
	witness and shuffle witness. We only need to focus on the omega witness. The
	existence of a omega witness means there is a omega sequence of factors, each
	evaluating to $a^{\omega^i}$. Since we do not have a formula for $a^{\omega^i}$,
	we instead use the formula for the $\mathcal{J}$ class drop of the above element.
	By pigeon hole principle, there exists some $j \in \{0, i-1\}$ such that
	$\exists^{\omega^j} x . c(x)$ is true for infintely many of these factors. So,
	$\exists^{\omega^{j+1}} x. c(x)$ is true for words that are part of the
	$\mathcal{J}$ class drop. A disjunction over all $j$ and letter witness
	formulas provides us the $\mathcal{J}$ class drop sentence in necessary form. Note
	that any shuffle witness will also satisfy the omega witness formula. This
	completes the proof.
\end{proof}

For any countable word $u$, we define the $\omega$-rank of a letter $a$ in the word,
denoted $\omega$-$\mathrm{rank}(a,u)$, to be the maximum $n \in \mathbb{N} \cup \{0\}$
such that $a^{\omega^n}$ is a subordering in $u$. If this happens for every $n \in
\mathbb{N}$, we say $\omega$-$\mathrm{rank}(a,u) = \infty$. Similarly, $\omega^*$-rank is
defined.

\begin{lemma}\label{lem:rankcontent}
Let $M$ be a commutative, idempotent o-algebra with the following additional properties
\begin{itemize}
	\item $(x^\tau)^{\tau^*} = (x^{\tau^*})^\tau = x^{\tau^*}x^\tau$
	\item $(xy)^\tau = x^\tau y^\tau$
	\item $(xy)^{\tau^*} = x^{\tau^*} y^{\tau^*}$
	\item $\{x_1, \ldots, x_k\}^\kappa = \{x_1\}^\kappa \ldots \{x_k\}^\kappa$
	\item $sc \Rightarrow sh$
\end{itemize}
Let $h \colon \Sigma^\circ \to M$ be a morphism. Then for any countable word $u$, \[ h(u)
= \prod_{a \in \mathrm{alph}(u)} m_a^{\tau^{n_1}} m_a^{\tau^{*^{n_2}}} \] where $m_a =
h(a)$, $\omega$-$\mathrm{rank}(a,u) = n_1$ and $\omega^*$-$\mathrm{rank}(a,u) = n_2$. Note
that if $n_1$ is $\infty$, then $m_a^{\tau^\infty}$ is just the fixpoint of applying
$\tau$ on $m_a$. 
\end{lemma}
\begin{proof}
	For finite words, clearly the lemma holds. Now we prove that the algebra operators
	preserve the property.
	\paragraph*{Concatenation} Let $u$ and $v$ be two countable words. Then
	\[ h(u).h(v) = \prod_{a \in \mathrm{alph}(u)} m_a^{\tau^{n_1}}m_a^{\tau^{*^{n_2}}}
	. \prod_{b \in \mathrm{alph}(v)} m_b^{\tau^{p_1}}m_b^{\tau^{*^{p_2}}} \]
	where $h(a)=m_a$, $n_1 =
	\omega {\text -}\mathrm{rank}(a,u)$, $n_2 = \omega^*{\text -}\mathrm{rank}(a,u)$,
	$h(b) = m_b$,
	$p_1 = \omega {\text -}\mathrm{rank}(b,v)$, and $p_2 = \omega^*{\text -} 
	\mathrm{rank}(b,v)$. The interesting case is when $a \in \mathrm{alph}(u) \cap
	\mathrm{alph}(v)$. Note that, in any o-algebra, $m^{\tau^i}.m^{\tau^j} =
	m^{\tau^j}$ if $i <j$, because $m^{\tau^j} = ({m^\tau}^{j-1})^\tau = m^{\tau^{j-1}}
	({m^\tau}^{j-1})^\tau = {m^\tau}^{j-1}m^{\tau^j}$. Since $M$ is commutative and
	idempotent, ${m^\tau}^i {m^\tau}^j = {m^\tau}^k$ where $k = \mathrm{max}(i,j)$.
	The rest follows easily.
	
	\paragraph*{Omega} Let $u$ be a countable word. Then
	\[ h(u^\omega) = (h(u))^\tau = \left(\prod_{a\in \mathrm{alph}(u)}
			m_a^{\tau^{n_1}} m_a^{\tau^{*^{n_2}}} \right )^\tau
			= \prod_{a \in \mathrm{alph}(u)} m_a^{\tau^{n_1+1}}
			(m_a^{\tau^{*^{n_2}}})^\tau
		\]
	where the last equality follows from the property $(xy)^\tau = x^\tau
	y^\tau$. Using the property, $(x^\tau)^{\tau^*} = (x^{\tau^*})^\tau =
	x^{\tau^*}x^\tau$, we can see that for $m,n > 0$,
	$(x^{\tau^m})^{\tau^{*^n}} = (x^{\tau^{*^n}})^{\tau^m} =
	x^{\tau^{*^n}}x^{\tau^m}$.  Using idempotent and commutative property, we
	get $m_a^{\tau^{n_1+1}} (m_a^{\tau^{*^{n_2}}})^\tau = m_a^\tau
	m_a^{\tau^{n_1+1}} m_a^{\tau^{*^{n_2}}} = m_a^{\tau^{n_1+1}}
	m_a^{\tau^{*^{n_2}}}$. So the property is preserved. 

	\paragraph*{Omega-star} Similar to omega.

	\paragraph*{Shuffle}
	{\color{red}Claim without proof, probably wrong}: $x^{sc} \leq_{\mathcal{J}}
	x^\kappa \leq_{\mathcal{J}} (x^{sc})^\kappa$ for any o-monoid.

	Since $x^{sc} = (x^{sc})^\kappa$ and every $\mathcal{J}$-class can have only one
	shuffle idempotent, we get $x^\kappa = x^{sc}$. Also by the properties of $M$, the
	operation sc results in $x^{sc} = x^{\tau^\infty}x^{\tau^{*^\infty}}$.

	Let $u_1, u_2, \ldots, u_k$ be countable words. Then
	\[ h(\{u_1, \ldots, u_k\}^\eta) = \{h(u_1), \ldots, h(u_k)\}^\kappa 
	= (h(u_1))^\kappa \ldots ((h(u_k))^\kappa \]
	The rest follows easily.
\end{proof}

\begin{theorem}\label{thm:gfo-one}
Let $L \subseteq \Sigma^\circ$ be a language. Then the following are equivalent.
\begin{enumerate}
	\item $L$ is recognized by a commutative idempotent monoid with $sc \Rightarrow
		sh$, and other properties of Lemma~\ref{lem:rankcontent}.
	\item $L$ is definable in $GFO^1$.
	\item $L$ is recognized by direct products of $\Omega_n$ and $\Omega^*_n$ for some
		$n \in \mathbb{N}$.
\end{enumerate}
\end{theorem}

\begin{theorem}
	$\fo[\eo{n}, \eos{n}] \equiv \Box^* {\alo{n}, \alos{n}}$
\end{theorem}
\begin{proof}
	We only prove the first item.

	($\Leftarrow$) The proof is via induction on number of elements in a block
	product. Base case is done by Lemma~\ref{lem:singleomega}.

	Suppose $M$ is an algebra that recognizes languages expressible in this logic.
	Then $L \subseteq \Sigma^\circ$, recognized by $M \Box \Omega_n$, is a boolean
	combination of languages like $L_1 \subseteq \Sigma^\circ$ recognized by $M$ and
	$L_2 \subseteq (M \times \Sigma \times M)^\circ$ recognized by $\Omega_n$. If
	$\sigma$ is the transducer (from the block product principle), then by
	Lemma~\ref{lem:singleomega} we only need
	to express $\sigma^{-1}(L_2)$ in the generalized FO logic when $L_2$ is expressed
	as $\exists^{\omega^i}x.(m_1,c,m_2)(x)$. Quite clearly, $w \models
	\exists^{\omega^i}x.(\phi_{m_1}|_{<x} \land c(x) \land \phi_{m_2}|_{>x})$ if and
	only if $\sigma(w) \models \exists^{\omega^i}x.(m_1,c,m_2)(x)$.

	($\Rightarrow$) This direction of the proof goes via induction on formula of the
	new logic. The only cases we need to show are the new quantifiers. 

	Let $\phi = \exists^{\omega^i} \psi$ be a formula where $L(\psi) \subseteq (\Sigma
	\times \{0,1\})^\circ$ is inductively recognized by $h \colon (\Sigma \times
	\{0,1\})^\circ \to M$, that is, there is a set $F \subseteq M$ such that 
	$h^{-1}(F) = L(\psi)$. We prove that $M \Box \Omega_n$ recognizes $L(\phi)$.

	We show this by giving two morphisms $h_1 \colon \Sigma^\circ \to M$ and $h_2
	\colon (M \times \Sigma \times M)^\circ \to \Omega_n$. Let $h_1(c) = h((c,0))$ and
	suppose $h_2((m_1,c,m_2))$ equals $a^{\omega^0}$ if $m_1.h((c,1)).m_2 \in F$, and
	it equals $1$ otherwise. It is easy to see that $w \models \phi$ if and only if
	$h_2(\sigma(w)) \in \{ a^{\omega^i} , \ldots , a^{\omega^n} \}$.
\end{proof}
\begin{corollary}
Following characterizations follow.
\begin{itemize}
   \item $\mathrm{FO}[\exists^\omega_\mathbb{N}] \equiv \Box^* \cup_{i \geq 1} \Omega_i$
   \item $\mathrm{FO}[\exists^{\omega^n},\exists^{\omega*^n}] \equiv \Box^*\{\Omega_n,
	   \Omega^*_n \}$
\end{itemize}
\end{corollary}

Block product characterizations allow us to show following logic inclusions.

\begin{theorem}
\begin{enumerate}
	\item $\mathrm{FO}[\exists^{\delta^n}] \subsetneq
		\mathrm{FO}[\exists^{\delta^{n+1}}]$. Similarly for the other quantifiers.
	\item $\mathrm{GFO} \subsetneq \mathrm{FO-cut}$.
	\item $\mathrm{FO}[\exists^{\delta^n}] \subsetneq \mathrm{FO}[\exists^{\omega^n},
		\exists^{\omega^{*^n}}]$
\end{enumerate}
\end{theorem}
\begin{proof}
	(1) By our equation hierarchy (next section). Should rewrite the way these
	equations are presented so that it does not take too much focus. Also we should
	probably just call it parameterized equations, and not use the term `equation
	hierarchy'. 

	(2) $e \mathcal{J} e^\tau \mathcal{J} e^{\tau^*} \implies e = e^\tau  e^{\tau^*}$
	Again have to show closure properties of this equation (division, direct product
	and block product). Gap monoid is the counter-example.

	(3) {\color{red}Unsure, but I believe this is true. I'll think about it.}
\end{proof}

\section{Equations Hierarchy}
For any o-monoid $M$, let us define a sequence of sets $(E_i(M))_{i \in
\mathbb{N}}$ as follows.
\begin{itemize}
    \item $E_0(M) = E(M)$ 
    \item $E_n(M) = \{(e^\tau e^{\tau*})^* \mid e \in E_{n-1}(M)\}$.
\end{itemize}
\begin{lemma}\label{lem:id-seq-morph}
    Let $h \colon M \to N$ be a surjective o-monoid homomorphism.
    \begin{enumerate}
        \item[(i)] If $e \in E_n(M)$, then $h(e) \in E_n(N)$.
        \item[(ii)] For any $e \in
    E_n(N)$, there exists $f \in h^{-1}(e) \cap E_n(M)$.
    \end{enumerate}
\end{lemma}
\begin{proof}
    (i). 
    For the base case, suppose $e \in E_0(M)$. Then $h(e) = h(e.e) = h(e).h(e)$.
    So $h(e) \in E_0(N)$. 

    For the induction step, suppose $e \in E_n(M)$. So $e =
    (f^\tau.f^{\tau^*})^*$ where $f \in E_{n-1}(M)$. By induction hypothesis,
    $h(f) \in E_{n-1}(N)$. Then $h(e) = ({h(f)}^\tau {h(f)}^{\tau^*})^*$.
    So $h(e) \in E_n(N)$. 

    (ii). For the base case, suppose $e \in E_0(N)$. Since $h$ is surjective, there
    exists $x \in M$ such that $h(x)=e$. Now $x$ may not be an idempotent, but
    note that $h(x^2) = h(x).h(x) = e.e =e$. So if $x^*$ is the idempotent power
    of $x$, then $h(x^*) = e$ and $x^* \in E_0(M) \cap h^{-1}(e)$. 

    For the induction step, suppose $e \in E_n(N)$. So $e =
    (f^\tau.f^{\tau^*})^*$ where $f \in E_{n-1}(N)$. By induction hypothesis,
    there is $f' \in h^{-1}(f) \cap E_{n-1}(M)$. Let $e' = ({f'}^\tau
    {f'}^{\tau^*})^*$. Then $h(e') = (f^\tau f^{\tau^*})^* = e$. So $e' \in E_n(M)
    \cap h^{-1}(e)$. 
\end{proof}

We now define a sequence of equations $(\mathbf{GI}.i)_{i \in \mathbb{N}}$ where
$\mathbf{GI}.n$ states for any o-monoid $M$ that all elements of $E_n(M)$ are
gap insensitive

\begin{lemma}\label{lem:eq-identity}
For any $n$, the equation $\mathbf{GI}.n$ is preserved under division and direct product.
\end{lemma}
\begin{proof}
    Suppose a monoid $M$ satisfies $\mathbf{GI}.n$. Consider a submonoid $N$ of $M$. We
    want to show $N$ also satisfies the equation. Let $e \in E_n(N)$. So $e = (f^\tau
    .f^{\tau^*})^*$ where $f \in E_{n-1}(N)$. By induction hypothesis, $f \in
    E_{n-1}(M)$. Hence $e \in E_n(M)$. Since $M$ satisfies $\mathbf{GI}.n$, the
    idempotent $e$ is gap insensitive. That is, $e = e^\tau.e^{\tau^*}$. Since
    $e^\tau$ and $e^{\tau^*}$ both belong in $N$ due to closure, it means $e$ is
    gap insensitive in $N$ as well. So, $N$ also satisfies $\mathbf{GI}.n$.

    Now suppose $M$ satisfies $\mathbf{GI}.n$ and $N$ is a homomorphic image of $M$ under
    $h \colon M \to N$. We want to show $N$ also satisfies $\mathbf{GI}.n$. Let $e \in
    E_n(N)$. By Lemma~\ref{lem:id-seq-morph}, there exists $f \in E_n(M)$ such
    that $h(f) = e$. Since $M$ satisfies $\mathbf{GI}.n$, we know that $f^\tau.f^{\tau^*}
    = f$ in $M$. But this means $h(f) = e$ is gap insensitive in $N$. So $N$
    also satisfies $\mathbf{GI}.n$.

    For direct product, it's easy to show by induction that $(e,f) \in E_n(M
    \times N)$ implies $e \in E_n(M)$ and $f \in E_n(N)$. The result then
    follows.
\end{proof}
We now show that the equations are preserved under block product of aperiodic
o-monoids. But first we need the following lemma.
\begin{lemma}
	Let $(m,f) \in E_n(M \Box N)$. Then $m \in E_n(M)$. Further, if 
        $M$ is aperiodic, then $m \ast f \ast m \in E_n(N^{M \times M})$.
\end{lemma}
\begin{proof}
    We prove this by induction. Base case is $n = 0$. Suppose $(m,f) \in E_0(M
    \Box N)$. This simply means that $(m,f)$ is an idempotent and hence $(m,f) =
    (m,f).(m,f)$. Now $(m,f).(m,f) = (m^2, f \ast m + m \ast f)$. This implies
    $m = m^2$ , that is, $m \in E_0(M)$. Also, 
    \begin{align*}
        f &= f \ast m + m \ast f \\
        \implies m \ast f \ast m &= m \ast f \ast m + m \ast f \ast m 
        ~[\because m.m =m ]
    \end{align*}
    So, $m \ast f \ast m \in E_0(N^{M \times M})$.

    For the induction step, let $e = (m_1,f_1) \in E_{n-1}(M \Box N)$ such that
    $(m,f) = (e^\tau e^{\tau*})^*$. Since $e$ is an idempotent, recall that
    $e^\tau = ({m_1}^\tau, f_1 \ast {m_1}^\tau + (m_1 \ast f_1 \ast {m_1}^\tau)^{\hat{\tau}})$ and
    $e^{\tau*} = ({m_1}^{\tau*}, ({m_1}^{\tau*} \ast f_1 \ast m_1)^{\hat{\tau*}}
    + {m_1}^{\tau*} \ast f_1)$.

    Let $(m',f') = e^\tau e^{\tau*}$. So $m' = {m_1}^\tau {m_1}^{\tau*}$ and 
	$f' = f_1 \ast m' + (m_1 \ast f_1 \ast m')^{\hat{\tau}}$
	$ + (m' \ast f_1 \ast m_1)^{\hat{\tau*}} + m' \ast f_1$. 
	Note that, $(m,f) = (m',f')^*$.

    Hence $m = m'^* = ({m_1}^\tau {m_1}^{\tau*})^*$. By induction, $m_1 \in E_{n-1}(M)$. 
	So, $m \in E_n(M)$. 

    Assuming the index of $(m',f')$ to be $k$, we get 
    \[f = \sum_{i=0}^{k-1} m'^i \ast f' \ast m'^{k-i-1}\]

    Using the aperiodicity of $M$, we know ${m'}^j = {m'}^k = m$ for any $j \geq k$.
    So we get the following implication.
    \[ m \ast f \ast m = (m \ast f' \ast m)^k \]
	
    Since $m \ast f \ast m$ is idempotent in $N^{M \times M}$ by similar
    argument as in the base case, we get
    \[ m \ast f \ast m = (m \ast f' \ast m)^* \]
        
    Again using aperiodicity of $M$, it's easy to check that
	$m \ast f' \ast m = (m \ast f_1 \ast m)^{\hat{\tau}} $ 
	$ + (m \ast f_1 \ast m)^{\hat{\tau*}}$. Since 
	$m \ast f_1 \ast m = m \ast (m_1 \ast f_1 \ast m_1) \ast m$
	and by induction hypthesis, $(m_1 \ast f_1 \ast m_1)^* \in E_{n-1}(N^{M \times M})$,
	we get that $(m \ast f_1 \ast m) \in E_{n-1}(N^{M \times M})$.
	Hence $m \ast f \ast m \in E_n(N^{M \times M})$.
\end{proof}


\begin{theorem}
	The equations $(\mathbf{GI}.n)_{i \in \mathbb{N}}$ are all preserved
	under block product of aperioidc o-monoids.
\end{theorem}
\begin{proof}
	Consider two o-monoids $M$ and $N$ that both satisfy equation $\mathbf{GI}.n$
    and let $M$ be aperiodic.
	We prove that $M \Box N$ also satisfy the equation.

	Let $e = (m,f) \in E_n(M \Box N)$. Then 
$		e^\tau e^{\tau*}  =  (m^\tau m^{\tau*}, f \ast m^\tau m^{\tau*}
		+ (m \ast f \ast m^\tau m^{\tau*})^{\hat{\tau}} 
		+ (m^\tau m^{\tau*} \ast f \ast m)^{\hat{\tau*}} + m^\tau m^{\tau*} \ast f) $.
		By previous lemma, $m^\tau m^{\tau*} = m$ and $(m \ast f \ast m)^{\hat{\tau}}
		+ (m \ast f \ast m)^{\hat{\tau*}} = m \ast f \ast m$. Thus
		$e = e^\tau e^{\tau*}$. 
\end{proof}

\begin{corollary} FO-CUT cannot have a block product characterization using any
finite set of o-monoids.  \end{corollary} 

\begin{proof} 
    Suppose a finite
    set of aperiodic o-monoids under block product closure and division exactly
    correspond to o-monoids recognizing FO-CUT languages. Since any o-monoid is
    finite, there is a $m \in \mathbb{N}$ such that for all $n > m$, the
    equations $\mathbf{GI}.n$ are satisfied by the o-monoids in the set.  Then
    this continues to be the case in the block product closure of the set.
However the chain $I_n$ belongs in FO-CUT and cannot belong in this closure.
Hence, we get a contradiction.
\end{proof} 


==> conclusion.tex <==
In this paper we saw blah blah blah.
